Mining actionable information from security forums: the case of malicious IP addresses

The goal of this work is to systematically extract information from hacker forums, whose information would be in general described as unstructured: the text of a post is not necessarily following any writing rules. By contrast, many security initiatives and commercial entities are harnessing the readily public information, but they seem to focus on structured sources of information. Here, we focus on the problem of identifying malicious IP addresses, among the IP addresses which are reported in the forums. We develop a method to automate the identification of malicious IP addresses with the design goal of being independent of external sources. A key novelty is that we use a matrix decomposition method to extract latent features of the behavioral information of the users, which we combine with textual information from the related posts. A key design feature of our technique is that it can be readily applied to different language forums, since it does not require a sophisticated Natural Language Processing approach. In particular, our solution only needs a small number of keywords in the new language plus the users behavior captured by specific features. We also develop a tool to automate the data collection from security forums. Using our tool, we collect approximately 600K posts from 3 different forums. Our method exhibits high classification accuracy, while the precision of identifying malicious IP in post is greater than 88% in all three forums. We argue that our method can provide significantly more information: we find up to 3 times more potentially malicious IP address compared to the reference blacklist VirusTotal. As the cyber-wars are becoming more intense, having early accesses to useful information becomes more imperative to remove the hackers first-move advantage, and our work is a solid step towards this direction.

==> 240-usersroles.tex <==
\section{Identifying users roles}
\label{sec:userroles}
   \textbf{behavioral analysis} \\* 
   We propose a systematic approach to identify the group of users discuss more about malicious activities or raise more anxiety in the forum. First we need to figure out different roles of the users in terms of their behavioral activity in the forum. To fulfill this goal, we utilize a hard coclustering method. Consequently, based on the proposed features in \reminder{\ref{ufeat}}, we find 5 major behavioural characteristics. \reminder{why using coclustering be helpful and the intuition behind using coclustering instead of traditional clustering like K means}.

  Having these unsupervised clustering result help us interpret better users' behavior and select a part of the users based on their participation behavior in the thread. Therefore, we can do appropriate actions regarding to each role.
   
    \begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth,height=5cm]{timeserie2}
    \caption{test fig}
    \label{fig:timeSeries}
    \end{figure*}

  Information theoretic as a hard Co-clustering methods raise five different behavior that we can call them, \textit{HeavyHitters}, \textit{Consumers},  \textit{High producers}, \textif{Average producers},  \textit{Minimum producers} ina bigger group we put last three as \PR. \HH are the group of users who their activities in all aspects are in the highest rate. \CS are the group of users who has the lowest participation rate, fewest number of posts, threads, etc and another main characteristics of these users is that they participate mostly in a threads created by themselves. In other words, they initiate a discussion then after probably getting their answers then have no more participation. Therefore, in this way, they also have low thread entropy. \HP are the group of users who are not as active as \HH but they have high value as day and thread entropy and they posted large number of post. \AP and \LP are similar to \HP in terms of having large number of post and participate in more thread than \CS but their entorpies are not as high as \HP. 
  \reminder{I am not sure that the following is well supported Kostas do you suggest any why to justify it?} Knowing about the users roles will provide us the knowledge to see which kind of the users and their activity should be highly monitored in security forums. To elaborate more on this we will consider \WS and \Offcomm as the selected datasets for the rest of paper. In all monitored security forum, people use words like \textit{\{Help,Trouble,Scary,freak out, Panic, problem, etc\}} to describe about their anxiousness relating to an attack or effect of a malware or virus on their machines. \Therefore, as a simplification if we suppose using these terms in a text means the topics of the talk is about malware and anxiety. First, We can say that considering the frequency of these term leads to the point of interest.Second, people bring their questions and problems in to attention of forums experts  by initiating a thread and talking about their issue. To this end, we need to see who has initiated a thread and discuss about it's fear of a malware or report these terms in a thread.
  
  Considering the different user's roles and initializing a discussion and talking about point of interest we can have different questions in these research that we will consider two in following:
  \\ \textit{1) Which group of users have more concerns about malware and bring up more related topics?}
  \\ \textit{2) Which group of users follow the malware related concern in the forum and provide more information about them or give answers to the questions?} 
  \reminder{\PR is the answer for both}
  
  To address the first hypothesis, we investigate the correlation between number of threads initiated in the forum and those are talking about subjective concerns on malicious activities. Therefore, we propose a list of keywords in two categories namely, \textit{Malware} jargon and \textit{Anxiety} jargon. The list of these words can be seen in the table \ref{tbl:keywords}.
  By monitoring the existence of these words and all their stems in initialized threads, we observe that \PR inject more malware related anxiety into forum discussions. Figure \ref{fig:timeSeries} depicts the noticeable correlation in the group of producers in 2009. In terms of quantitative analysis, the Pearson correlation coefficient \cite{????} also implies that this value is drastically larger in group of the producers than other users' roles.




 \begin{table}
 \centering 
 \begin{tabular}{| c | c | c | c | c|} 
 \hline
 {} &  \multicolumn{2}{c|}{WildersSec.} & \multicolumn{2}{c|}{OffensiveComm.}    \\ 
 \hline
 Dataset & \Rho & \pvalue & \Rho & \pvalue \\ 
 \hline
 \CS & 0.60 & 2.51E-145 & 0.51 &  1.38E-40 \\ 
 \hline
 \HH & 0.14 & 0.02 & \textbf{0.76} & 8.42E-51 \\
 \hline
 Others & \textbf{0.61} & 1.57E-133 & \textbf{0.68} & 2.08E-57 \\
 \hline
\end{tabular}
\caption {Pearson correlation coefficient for \WS and \OffComm over 4 years from 2012 to 2015}
\end{table}
   
 Consequently, even though we expected \CS' posts imply more anxiety relating to malware. By considering the correlation of initialized thread and usage of two sets of keywords separately we will notice that even though the \CS talk more about their anxieties by using listed keywords but lower correlation coefficient in malware related keywords is the reason of placing in the second order of groups of users talk about the both together. However, \PR's correlation coefficient implies the first group of the users who talks about related topics is this group. However, \HH who we generally define as the group of people with higher activity in \WS, based on the correlation coefficient, are not reacting anxiously to malwares. On the other hand, in offensive community most of threads in the point of interest are generated by \HH. The reason for this happening is in \OffComm \reminder{XXX} percent of the post initialized and \reminder{XXX} of the post has been writing by this group of people. 
 \reminder{conclusion}\\This findings show that the answer to the first question is \PR. Accordingly, in terms of security related issue by monitoring these group of users more points of interest will be observed.
 
 \begin{table}
 \centering 
 \begin{tabular}{| p{1cm} | m{7cm} |} 
 \hline
 Category & Keywords \\
 \hline
 Malware &   spyware, adware,	scareware, ransomware,	keystroke,	keylogging,	rootkit,	trojan,	virus,	worm,	backdoor,	botnet,	hijack,	overflow,	exploit,	honeypot,	patch,	phishing,	spam,	spoofing,	sql, injection,	injection,	zombie,	attack,	XSS,	zero-day,	Antivirus (AV),	vendor.
  \\ 
 \hline
 Anxiety & fear	panic,	worry,	care,	angst,	stress,	concern,	suspense,	freak out,	bother,	horror,	terror,	alarm,	pain,	problem,	trouble,	help,	warn,	help,	aid,	horrible,	terrify,	frighten,	scary,	difficulty,	hard,	chilling,	shivery,	suspect,	suspicious.
 \\ 
 \hline
\end{tabular}
\caption {List of keywords}\label{tbl:keywords}
\end{table}
 
Not only initializing a discussion and starting a question which we investigate in the first question \reminder{is important} but also following an initiated thread in the point of intrests topic indicates which parts of the thread should be observe to gain more. In that vain, in other to address the second question, we discriminate between the first and the other posts that users publish in the threads. Then, we will investigate based on the used keywords in the first post what would be in the following in term of the users roles and discussion that they bring up. Here, we again consider two jargons of keyword mentioned in table \ref{tbl:keywords}. It is worth to mentioning that in order to diminish the effect of number of post in each thread, we consider the number of thread in which keywords from either those categories appear as a first or following posts. \reminder{more description}

 
 \begin{figure}
  \centering
  \subfloat[malware usage]
  {\includegraphics[width=0.5\linewidth]{Fol_CS_mal}\label{fig:f1}}
  \hfill
  \subfloat[anxiety usage]
  {\includegraphics[width=0.5\linewidth]{Fol_CS_anx}\label{fig:f2}}
  \caption{keyword usage by group of users following Consumers in \WS}\label{fig:Fol_CS}
\end{figure}
 


 \begin{figure}[!tbp]
  \centering
  \subfloat[malware usage]
  {\includegraphics[width=0.5\linewidth]{Fol_HH_mal}\label{fig:f1}}
  \hfill
  \subfloat[anxiety usage]
  {\includegraphics[width=0.5\linewidth]{Fol_CS_anx}\label{fig:f2}}
  \caption{keyword usage by group of users following Heavy-Hitter in \WS}\label{fig:Fol_HH}
\end{figure}


 \begin{figure}[!tbp]
  \centering
  \subfloat[malware usage]
  {\includegraphics[width=0.5\linewidth]{Fol_PR_mal}\label{fig:f1}}
  \hfill
  \subfloat[anxiety usage]
  {\includegraphics[width=0.5\linewidth]{Fol_PR_anx}\label{fig:f2}}
  \caption{keyword usage by group of users following Producers in \WS}\label{fig:Fol_PR}
\end{figure}

As it can be seen in figure \ref{fig:Fol_CS} and \ref{fig:Fol_HH} in the both cases \PR disregard to the topic of discussion have higher rate of following. Moreover, \CS and \HH have a homophily in the case of following an initiated thread. It means that people in these groups tends to follow the threads which are initialized by a member of their cluster. For example, in figure \ref{fig:Fol_HH} \HH follow in 35\% of the thread that initialized with other \HH and discuss about malwares similarly in 38\% of the thread they follow with anxiety keywords, comparing to the small value for \CS's following we can observe the homophily in followers.\reminder{any thought any HELP}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{j_userclusterWilder}
    \caption{\reminder{User clustering visualization: the intensity of the average value of each features in the cluster are normalized to show it is closer to maximum, minimum or mean value, respectively shows 1,2,3 as the level, of that feature}}
    \label{fig:userCluster}
\end{figure*}

==> makefile <==
TARGET=paper
LATEX=pdflatex

all:  
	${LATEX} ${TARGET}.tex
	bibtex ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex

#	dvips -t letter ${TARGET}.dvi -o ${TARGET}.ps
#	ps2pdf ${TARGET}.ps ${TARGET}.pdf


clean:
	\rm -f *.dvi *.bbl *.log *.aux *.blg *.bak *.db *.out *.ps *.pdf
	\rm -f $(MAIN).ps $(MAIN).pdf $(MAIN).dvi
	\rm -f paper.pdf

spotless: clean
	\rm -rf TST all.tar


==> related.tex <==
\section{Related Works}

